Transit drivers' reflections on the benefits and harms of eye tracking technology

Eye tracking technology offers great potential for improving road safety. It is already being built into vehicles, namely cars and trucks. When this technology is integrated into transit service vehicles, employees, i.e., bus drivers, will be subject to being eye tracked on their job. Although there is much research effort advancing algorithms for eye tracking in transportation, less is known about how end users perceive this technology, especially when interacting with it in an employer-mandated context. In this first study of its kind, we investigated transit bus operators' perceptions of eye tracking technology. From a methodological perspective, we introduce a mixed methods approach where participants experience the technology first-hand and then reflect on their experience while viewing a playback of the recorded data. Thematic analysis of the interview transcripts reveals interesting potential uses of eye tracking in this work context and surfaces transit operators' fears and concerns about this technology.

==> Sections/6_Conclusion.tex <==
\section{Conclusion}


\appendix
\section{Appendix: NASA TLX}
\shaina{Are we allowed an Appendix? On the submission form, there is this text: Please ensure that no content (except references), including figures, tables, body text, or acknowledgments, flows onto the 9th page. Can we possibly attach as supplemental material? Text from the submission form: Use this space to include supplementary material, such as videos, datasets, results, etc. For videos, we recommend MP4 format with H.264 codec. Supplementary materials will be reviewed for quality and acceptability for inclusion in the ACM digital library and conference proceedings. As with the paper submission, the supplemental material needs to be blinded for peer review. Note: All supplemental materials will be visible to all reviewers!} 
\ejain{Ok, let's do the following: we can move this to supplementary for the submission, but for the author preprint (which we put on our website) let's have it as Appendix.}

The NASA TLX items were as follows, where the initial question would be asked, and if the subject demonstrated any confusion, the supplemental clarifying questions would be asked: 
Mental Demand: How mentally demanding was wearing the eye-tracking glasses?
(0 is not demanding, 10 is very demanding)
How much mental and perceptual activity was required?
Was the task easy or demanding, simple or complex?
Physical Demand: How mentally demanding was wearing the eye-tracking glasses?
(0 is not demanding, 10 is very demanding)
How much physical activity was required?
Was the task easy or demanding, slack or strenuous?
Temporal Demand: How hurried or rushed was the pace of driving with the eye-tracking glasses on?
(0 is not hurried or rushed, 10 is very demanding)
How much time pressure did you feel due to the pace at which the tasks occurred?
Was the pace slow or rapid?
Overall Performance: How successful were you in driving with the eye-tracking glasses on?
(0 is not successful, 10 is very successful)
How successful were you in performing the task?
How satisfied were you with your performance?
Note that this question was not asked in the conventional method (10 is not successful, 0 is very successful) to avoid confusing the drivers. The research team found this to be confusing and asked the question in the above manner, then reversed the scores for total TLX score calculation (i.e. a 10 became a 0, a 1 became a 9, a 9.5 became a 0.5, etc.) 
Effort: How hard did you have to work (mentally and physically) to accomplish your level of performance?
(0 is not hard, 10 is very hard)
Frustration Level: How irritated, stressed, and annoyed versus content, relaxed, and complacent did you feel during the task?
(0 is content, relaxed, and complacent, 10 is irritated, stressed, and annoyed)
